SCAR: Bridging Coarse Retrieval and Fine Localization through Candidate Reranking

Natural-language point-cloud localization typically retrieves candidate map cells and then predicts a position inside each candidate, yet the final output is still determined by retrieval order. A retrieval score measures region-description relevance, not whether the coordinates a region yields are accurate: a relevant region may produce a displaced prediction, and a lower-ranked region may contain a successful one. We study the final selection problem after the candidate pool and Fine predictions are fixed---how to choose the coordinate most likely to localize successfully, and under which conditions the gain holds. We propose SCAR (Spatial Consistency-Aware Reranking). SCAR treats each cell--Fine-coordinate pair as a localization hypothesis, interprets directional relations as functions of position, and reads spatial support at the backbone's actual Fine point (Fine-conditioned Evidence Readout). It organizes this readout with center support, semantic presence, retrieval score, and geometric offsets into a 23-D representation, trains a shared scorer with localization-success labels, and at inference reranks existing hypotheses and returns their original coordinates. Experiments cover four public backbones and a corrected Des4Pos reimplementation across five domains. Excluding one protocol-reference configuration, exploratory TEST point estimates on the remaining 24 configurations show Top-1@5\,m above Original on 23 and Cell R@1 above Original on all 24. On development-set VAL, the Fine readout improves Top-1@5\,m by 5.77 percentage points (pp) over a center surrogate on corrected Des4Pos*KITTI, and the complete scoring scheme improves it by 13.98\,pp over FSR on MambaPlace$\times$nuScenesFull; the latter measures the complete scheme, not learned ranking alone.

==> controls.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llcccc@{}}
\toprule
Dataset & Backbone & Presence & Rank Fusion & FSR & SCAR \\
\midrule
KITTI & Text2Loc & 49.05 / 41.28 & 54.58 / 44.62 & 58.65 / 46.51 & 59.45 / 43.74 \\
 & Text2Loc++ & 56.45 / 44.98 & 59.05 / 46.05 & 63.36 / 47.51 & 64.15 / 45.02 \\
 & MNCL & 54.90 / 46.01 & 57.56 / 46.62 & 62.00 / 48.19 & 63.82 / 47.41 \\
 & MambaPlace & 45.31 / 35.74 & 53.72 / 42.36 & 57.65 / 44.18 & 57.07 / 40.83 \\
 & Des4Pos (reimpl.) & 46.03 / 36.71 & 53.01 / 42.67 & 57.41 / 44.37 & 57.84 / 43.11 \\
\addlinespace[2pt]
S3DIS & Text2Loc & 28.23 / 29.89 & 36.90 / 38.38 & 44.83 / 46.49 & 41.33 / 41.70 \\
 & Text2Loc++ & 32.10 / 34.32 & 38.56 / 40.41 & 45.20 / 47.42 & 45.94 / 48.15 \\
 & MNCL & 28.97 / 30.26 & 34.69 / 35.79 & 37.64 / 38.93 & 38.38 / 39.30 \\
 & MambaPlace & 29.52 / 31.92 & 35.42 / 37.08 & 37.45 / 39.30 & 40.77 / 42.25 \\
 & Des4Pos (reimpl.) & 30.44 / 33.03 & 34.32 / 36.16 & 38.38 / 40.41 & 37.82 / 39.11 \\
\addlinespace[2pt]
PandaSet & Text2Loc & 48.75 / 52.95 & 43.75 / 46.75 & 40.50 / 43.10 & 44.95 / 52.35 \\
 & Text2Loc++ & 42.30 / 47.30 & 41.25 / 44.85 & 37.90 / 41.35 & 44.30 / 49.10 \\
 & MNCL & 30.25 / 34.10 & 35.10 / 38.75 & 35.40 / 38.95 & 42.05 / 47.85 \\
 & MambaPlace$^{\dagger}$ & 19.85 / 28.85 & 22.30 / 30.90 & 24.15 / 31.75 & 22.15 / 29.50 \\
 & Des4Pos (reimpl.) & 29.50 / 40.00 & 32.15 / 41.80 & 30.45 / 37.30 & 31.55 / 41.55 \\
\addlinespace[2pt]
nuScenes & Text2Loc & 50.93 / 58.08 & 47.26 / 54.22 & 42.58 / 49.01 & 54.68 / 62.19 \\
 & Text2Loc++ & 51.20 / 58.72 & 47.21 / 54.60 & 44.32 / 51.30 & 53.36 / 60.56 \\
 & MNCL & 41.36 / 52.74 & 35.54 / 45.90 & 32.18 / 41.66 & 52.47 / 65.28 \\
 & MambaPlace & 41.15 / 53.24 & 36.44 / 47.08 & 33.32 / 42.46 & 47.71 / 60.11 \\
 & Des4Pos (reimpl.) & 37.77 / 55.40 & 34.34 / 50.07 & 31.03 / 45.40 & 41.44 / 60.11 \\
\addlinespace[2pt]
NPM3D & Text2Loc & 27.59 / 33.62 & 27.59 / 33.62 & 27.59 / 33.62 & 26.72 / 31.03 \\
 & Text2Loc++ & 17.24 / 19.83 & 17.24 / 19.83 & 17.24 / 19.83 & 16.38 / 19.83 \\
 & MNCL & 9.48 / 13.79 & 9.48 / 13.79 & 9.48 / 13.79 & 14.66 / 19.83 \\
 & MambaPlace & 19.83 / 24.14 & 19.83 / 24.14 & 19.83 / 24.14 & 19.83 / 24.14 \\
 & Des4Pos (reimpl.) & 23.28 / 27.59 & 23.28 / 27.59 & 23.28 / 27.59 & 23.28 / 27.59 \\
\bottomrule
\end{tabular*}


==> localization.tex <==
 \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccccc@{}}
\toprule
 & \multicolumn{4}{c}{\textbf{KITTI}} & \multicolumn{4}{c}{\textbf{S3DIS}} & \multicolumn{4}{c}{\textbf{PandaSet}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
Backbone & 1\,m & 3\,m & \textbf{5\,m} & 10\,m & 1\,m & 3\,m & \textbf{5\,m} & 10\,m & 1\,m & 3\,m & \textbf{5\,m} & 10\,m \\
\midrule
Text2Loc & \SCARresult{6.46}{+3.36} & \SCARresult{37.16}{+16.68} & \SCARresult{59.45}{+24.31} & \SCARresult{75.77}{+26.88} & \SCARresult{30.26}{+20.85} & \SCARresult{39.30}{+27.31} & \SCARresult{41.33}{+27.49} & \SCARresult{41.70}{+27.31} & \SCARresult{7.70}{+0.15} & \SCARresult{30.85}{+2.30} & \SCARresult{44.95}{+4.00} & \SCARresult{55.25}{+4.75} \\
Text2Loc++ & \SCARresult{8.29}{+3.78} & \SCARresult{41.23}{+15.09} & \SCARresult{64.15}{+20.43} & \SCARresult{78.86}{+21.10} & \SCARresult{34.50}{+18.27} & \SCARresult{44.10}{+24.17} & \SCARresult{45.94}{+25.28} & \SCARresult{47.97}{+26.20} & \SCARresult{4.55}{+0.35} & \SCARresult{29.45}{+4.00} & \SCARresult{44.30}{+6.95} & \SCARresult{56.30}{+8.85} \\
MNCL & \SCARresult{7.20}{+2.83} & \SCARresult{40.40}{+11.26} & \SCARresult{63.82}{+14.23} & \SCARresult{79.69}{+13.99} & \SCARresult{22.88}{+18.08} & \SCARresult{36.90}{+29.70} & \SCARresult{38.38}{+30.44} & \SCARresult{39.11}{+31.18} & \SCARresult{4.65}{-0.30} & \SCARresult{27.20}{-2.10} & \SCARresult{42.05}{-0.15} & \SCARresult{52.50}{-0.10} \\
MambaPlace$^{\dagger}$ & \SCARresult{7.21}{+3.95} & \SCARresult{36.01}{+17.49} & \SCARresult{57.07}{+25.09} & \SCARresult{72.92}{+28.34} & \SCARresult{22.14}{+16.24} & \SCARresult{38.19}{+27.68} & \SCARresult{40.77}{+28.78} & \SCARresult{42.07}{+28.60} & \SCARresult{1.80}{+0.45} & \SCARresult{14.35}{+5.65} & \SCARresult{22.15}{+8.25} & \SCARresult{34.65}{+11.85} \\
Des4Pos (reimpl.) & \SCARresult{6.62}{+4.17} & \SCARresult{36.11}{+19.06} & \SCARresult{57.84}{+28.47} & \SCARresult{73.53}{+32.37} & \SCARresult{22.32}{+14.21} & \SCARresult{36.35}{+22.51} & \SCARresult{37.82}{+23.25} & \SCARresult{39.11}{+23.25} & \SCARresult{3.25}{+0.60} & \SCARresult{21.60}{+8.95} & \SCARresult{31.55}{+11.20} & \SCARresult{44.65}{+14.65} \\
\bottomrule
\end{tabular*}
\par\medskip
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccc@{}}
\toprule
 & \multicolumn{4}{c}{\textbf{nuScenes}} & \multicolumn{4}{c}{\textbf{NPM3D}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
Backbone & 1\,m & 3\,m & \textbf{5\,m} & 10\,m & 1\,m & 3\,m & \textbf{5\,m} & 10\,m \\
\midrule
Text2Loc & \SCARresult{19.10}{+2.54} & \SCARresult{37.67}{+6.36} & \SCARresult{54.68}{+10.05} & \SCARresult{62.43}{+11.63} & \SCARresult{7.76}{+1.72} & \SCARresult{24.14}{+6.03} & \SCARresult{26.72}{+6.90} & \SCARresult{30.17}{+6.90} \\
Text2Loc++ & \SCARresult{19.15}{+3.58} & \SCARresult{35.59}{+8.44} & \SCARresult{53.36}{+13.43} & \SCARresult{60.69}{+16.39} & \SCARresult{3.45}{0.00} & \SCARresult{14.66}{+6.03} & \SCARresult{16.38}{+6.90} & \SCARresult{19.83}{+8.62} \\
MNCL & \SCARresult{7.43}{+1.12} & \SCARresult{34.55}{+4.03} & \SCARresult{52.47}{+6.35} & \SCARresult{64.80}{+8.43} & \SCARresult{4.31}{+4.31} & \SCARresult{13.79}{+9.48} & \SCARresult{14.66}{+10.34} & \SCARresult{18.10}{+12.07} \\
MambaPlace & \SCARresult{7.24}{+0.49} & \SCARresult{31.68}{+4.38} & \SCARresult{47.71}{+7.04} & \SCARresult{60.21}{+9.66} & \SCARresult{4.31}{+0.86} & \SCARresult{15.52}{+2.59} & \SCARresult{19.83}{+2.59} & \SCARresult{24.14}{+3.45} \\
Des4Pos (reimpl.) & \SCARresult{6.27}{+0.26} & \SCARresult{23.79}{+3.24} & \SCARresult{41.44}{+5.42} & \SCARresult{59.76}{+8.28} & \SCARresult{0.00}{0.00} & \SCARresult{15.52}{+6.90} & \SCARresult{23.28}{+10.34} & \SCARresult{27.59}{+13.79} \\
\bottomrule
\end{tabular*}


==> retrieval.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccccc@{}}
\toprule
 & \multicolumn{4}{c}{\textbf{KITTI}} & \multicolumn{4}{c}{\textbf{S3DIS}} & \multicolumn{4}{c}{\textbf{PandaSet}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
Backbone & R@1 & R@3 & R@5 & R@10 & R@1 & R@3 & R@5 & R@10 & R@1 & R@3 & R@5 & R@10 \\
\midrule
Text2Loc & \SCARresult{43.74}{+13.90} & \SCARresult{70.00}{+19.85} & \SCARresult{76.99}{+16.82} & \SCARresult{81.33}{+10.01} & \SCARresult{41.70}{+27.31} & \SCARresult{63.84}{+32.10} & \SCARresult{72.51}{+25.83} & \SCARresult{85.42}{+20.66} & \SCARresult{52.35}{+7.30} & \SCARresult{77.40}{+5.20} & \SCARresult{85.40}{+2.40} & \SCARresult{92.90}{+2.80} \\
Text2Loc++ & \SCARresult{45.02}{+10.02} & \SCARresult{72.36}{+14.74} & \SCARresult{80.15}{+13.26} & \SCARresult{85.02}{+8.09} & \SCARresult{48.15}{+26.20} & \SCARresult{70.11}{+24.54} & \SCARresult{82.29}{+24.91} & \SCARresult{89.11}{+18.08} & \SCARresult{49.10}{+7.95} & \SCARresult{69.15}{+4.45} & \SCARresult{83.20}{+9.00} & \SCARresult{91.75}{+2.65} \\
MNCL & \SCARresult{47.41}{+3.51} & \SCARresult{76.62}{+9.77} & \SCARresult{84.19}{+9.38} & \SCARresult{88.80}{+5.77} & \SCARresult{39.30}{+31.18} & \SCARresult{60.15}{+38.38} & \SCARresult{68.82}{+35.06} & \SCARresult{77.86}{+25.46} & \SCARresult{47.85}{+1.80} & \SCARresult{74.20}{+5.95} & \SCARresult{82.45}{+5.10} & \SCARresult{89.55}{+2.50} \\
MambaPlace$^{\dagger}$ & \SCARresult{40.83}{+16.28} & \SCARresult{65.34}{+21.56} & \SCARresult{72.03}{+18.83} & \SCARresult{76.26}{+11.79} & \SCARresult{42.25}{+28.78} & \SCARresult{64.76}{+33.03} & \SCARresult{73.80}{+31.55} & \SCARresult{82.66}{+23.99} & \SCARresult{29.50}{+9.70} & \SCARresult{46.90}{+11.95} & \SCARresult{57.35}{+11.55} & \SCARresult{73.20}{+14.85} \\
Des4Pos (reimpl.) & \SCARresult{43.11}{+19.44} & \SCARresult{65.72}{+23.06} & \SCARresult{71.67}{+20.11} & \SCARresult{75.35}{+12.07} & \SCARresult{39.11}{+23.06} & \SCARresult{61.44}{+27.31} & \SCARresult{72.51}{+29.15} & \SCARresult{82.10}{+18.82} & \SCARresult{41.55}{+13.45} & \SCARresult{61.70}{+8.10} & \SCARresult{72.05}{+7.85} & \SCARresult{83.25}{+6.35} \\
\bottomrule
\end{tabular*}
\par\medskip
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccc@{}}
\toprule
 & \multicolumn{4}{c}{\textbf{nuScenes}} & \multicolumn{4}{c}{\textbf{NPM3D}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
Backbone & R@1 & R@3 & R@5 & R@10 & R@1 & R@3 & R@5 & R@10 \\
\midrule
Text2Loc & \SCARresult{62.19}{+11.58} & \SCARresult{76.31}{+9.78} & \SCARresult{81.16}{+7.32} & \SCARresult{87.42}{+4.39} & \SCARresult{31.03}{+6.90} & \SCARresult{53.45}{+9.48} & \SCARresult{76.72}{+15.52} & \SCARresult{95.69}{+16.38} \\
Text2Loc++ & \SCARresult{60.56}{+16.82} & \SCARresult{76.52}{+15.22} & \SCARresult{80.29}{+11.09} & \SCARresult{85.57}{+6.62} & \SCARresult{19.83}{+8.62} & \SCARresult{43.10}{+6.03} & \SCARresult{71.55}{+20.69} & \SCARresult{93.10}{+14.66} \\
MNCL & \SCARresult{65.28}{+8.97} & \SCARresult{81.26}{+8.59} & \SCARresult{86.82}{+6.27} & \SCARresult{91.61}{+4.11} & \SCARresult{19.83}{+13.79} & \SCARresult{45.69}{+22.41} & \SCARresult{62.93}{+25.86} & \SCARresult{95.69}{+39.66} \\
MambaPlace & \SCARresult{60.11}{+9.82} & \SCARresult{76.63}{+9.00} & \SCARresult{81.40}{+6.75} & \SCARresult{87.71}{+4.12} & \SCARresult{24.14}{+3.45} & \SCARresult{45.69}{+6.03} & \SCARresult{66.38}{+9.48} & \SCARresult{93.97}{+18.10} \\
Des4Pos (reimpl.) & \SCARresult{60.11}{+8.48} & \SCARresult{77.98}{+7.61} & \SCARresult{84.21}{+7.31} & \SCARresult{89.84}{+3.62} & \SCARresult{27.59}{+13.79} & \SCARresult{46.55}{+15.52} & \SCARresult{62.93}{+18.10} & \SCARresult{86.21}{+23.28} \\
\bottomrule
\end{tabular*}

